Limitless Regression Discontinuity

Conventionally, regression discontinuity analysis contrasts a univariate regression's limits as its independent variable, $R$, approaches a cut-point, $c$, from either side. Alternative methods target the average treatment effect in a small region around $c$, at the cost of an assumption that treatment assignment, $\mathcal{I}\left[R<c\right]$, is ignorable vis a vis potential outcomes. Instead, the method presented in this paper assumes Residual Ignorability, ignorability of treatment assignment vis a vis detrended potential outcomes. Detrending is effected not with ordinary least squares but with MM-estimation, following a distinct phase of sample decontamination. The method's inferences acknowledge uncertainty in both of these adjustments, despite its applicability whether $R$ is discrete or continuous; it is uniquely robust to leading validity threats facing regression discontinuity designs.

==> lrd-r1-concordance.tex <==
\Sconcordance{concordance:lrd-r1.tex:lrd-r1.Rnw:%
1 7 1 50 0 1 10 25 1 1 2 1 3 1 1 1 18 120 1 1 37 1 1 1 24 1 1 1 8 %
1 1 1 22 181 1 1 62 147 1 1 5 217 1 1 9 62 1 1 0 168 1}

